Coherent Spin Preparation of Indium Donor Qubits in Single ZnO Nanowires

Shallow donors in ZnO are promising candidates for photon-mediated quantum technologies. Utilizing the indium donor, we show that favorable donor-bound exciton optical and electron spin properties are retained in isolated ZnO nanowires. The inhomogeneous optical linewidth of single nanowires (60 GHz) is within a factor of 2 of bulk single-crystalline ZnO. Spin initialization via optical pumping is demonstrated and coherent population trapping is observed. The two-photon absorption width approaches the theoretical limit expected due to the hyperfine interaction between the indium nuclear spin and the donor-bound electron.

==> Sec1-Nanowire_SEM.tex <==
\section{Nanowire Ensemble Sample}
\label{Sec:Nanowire_SEM}
    \begin{figure}[!htbp]
  \centering
  \includegraphics[width=6in]{Figures/SI_Figures_SEM.png}
  \caption{\label{FigSI_1} 
  Scanning electron micrograph images of the ensemble nanowire sample (a) from directly above and (b) from a 45 degree angle.
  }
\end{figure}

==> Sec2-AB_PL.tex <==
\section{Nanowire Survey using Photoluminescence Spectra under above-band gap excitation}
\label{Sec:AB_PL}
Fig.~\ref{FigPL1} displays normalized photoluminescence spectra recorded on single dropcast nanowires and a nanowire ensemble. The excitation laser energy was 3.4440\,eV which is larger than the band gap of ZnO. Different single nanowires differ in the relative intensities of the surface exciton, Y-line, and In D$^0$-D$^0$X peak. Moreover, a broadening and splitting of the In D$^0$-D$^0$X and Y-line transitions can be observed for some single nanowires. This broadening and splitting is not observed in nanowire ensembles. Thus, we propose that the broadening and splitting of the In D$^0$-D$^0$X and Y-line transitions in the single nanowires is related to strain caused by the dropcasting process. In the main article, we mainly discuss results from nanowire~18, because it displays a In D$^0$-D$^0$X transition lineshape comparable to the nanowire ensemble sample.

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=5in]{Figures/NW_Overview.pdf}
  \caption{\label{FigPL1} 
  Photoluminescence spectra of several different dropcast nanowires (red, purple, and black) and the nanowire ensemble (blue). All measurements are normalized to the height of the In D$^0$-D$^0$X peak. All measurements are performed at 0\,T and 5.2\,K with an excitation laser energy of 3.4440\,eV. The excitation power was 36\,nW for the single nanowires and 10\,nW for the nanowire ensemble. The right panel is zoomed in to better observe the differences in the In D$^0$-D$^0$X peak. The line identifications are from~\cite{Meyer2004bed}.
  }
\end{figure}


==> Sec3-Res_Ext.tex <==
\section{Oscillatory Background Correction}

 A wavelength-dependent modulation of the signal is observed in single nanowire photoluminescence excitation (PLE) data. This is a consequence of a wavelength dependence of the transmittance and reflectance of the beamsplitter used in the excitation path. During the single nanowire measurements, the laser power was held constant at $P_\mathrm{C}$ (Fig.~\ref{FigMeasuredOscillation}b), leading to an oscillation in the excitation power, $P_\mathrm{A}$. In order to correct for this oscillation in the excitation power, the wavelength dependence of the ratio of the reflected to transmitted power for the beamsplitter was measured. Fig.~\ref{FigMeasuredOscillation}a shows a representative measurement. The wavelength dependence of $P_\mathrm{A}$/$P_\mathrm{B}$ was found to have minimal variation in offset, amplitude, and period, while the phase was found to change significantly between measurements, possibly depending on factors such as ambient temperature.

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=7in]{Figures/Measured_Oscillations.png}
  \caption{\label{FigMeasuredOscillation}  (a) A measurement of wavelength dependence of excitation path beamsplitter transmitted and reflected powers.  (b) Schematic of excitation path with power meter positions. 
  }
\end{figure}

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=7in]{Figures/Oscillation_Correction.png}
  \caption{\label{FigOscillationCorrection}  
  (a) Sine fit with fixed period for determination of oscillation phase from linear corrected background PLE intensity.  
  (b) Comparison of the phase and period of $P_\mathrm{A}$/$P_\mathrm{B}$ with low-energy background of the PLE intensity.  Two oscillations in the background can be seen to the left of the peak, matching the phase and period of the correction, shown in blue.
  (c,d) Example data from the measurement of CPT on the In D$^{0}$X in a single nanowire (c)~before and (d)~after correction. 
  }
\end{figure}

Correction of this oscillation was only applied to single-nanowire data where power was measured at $P_\mathrm{C}$ rather than $P_\mathrm{A}$. Assuming minimal absorption and scattering from the beamsplitter, and only phase changes in $P_\mathrm{A} / P_\mathrm{B}$, oscillations in the excitation power can be calculated. For simplicity, we will use \textit{f}(E, $\phi$) for handling $P_\mathrm{A} / P_\mathrm{B}$, using the data in Fig.~\ref{FigMeasuredOscillation} to define the function. $E$ is the excitation photon energy, and $\phi$ is the phase of the oscillation.

\[f(E, \phi) = \frac{\mathrm{P_A}}{\mathrm{P_B}} = 0.58 + 0.07\times \mathrm{sin}\left(\frac{2\pi E}{0.18 \mathrm{meV}} + \phi\right)\]


Minimal absorption and scattering tells us $\mathrm{P_C}$ = $\mathrm{P_A}$ + $\mathrm{P_B}$, thus $\mathrm{P_C}$ = $\mathrm{P_A}$ (1 + 1/\textit{f}(E, $\phi$)).  The mean power reflected over incident power $\mathrm{P_A} / \mathrm{P_C}$ is 0.36. 
This factor can be used to convert from an oscillating excitation power to a constant excitation power, as $\mathrm{P_C}$ was held constant during measurement. The oscillatory background correction is performed by determining the phase of \textit{f}(E, $\phi$), then multiplying the measured PLE intensity by the resulting energy dependent correction factor. 

\[\frac{\textrm{Corrected } \mathrm{P_A}}{\mathrm{P_A}} =(1 + \frac{1}{f(E, \phi)}) \cdot (0.36) = \textrm{Correction Factor}\]

In the regime where the PLE intensity is proportional to the probe power, PLE data can be accurately corrected using this factor. The probe power changes by 18$\%$ peak to peak. This small variation in excitation power from the oscillation allows for the approximation of the dependence of the PLE intensity on probe power as linear, Counts($E$) $\approx$ $\alpha P_\mathrm{A}$($E$) + $\beta$. For single-laser PLE and for two-laser PLE with observable oscillations in the off-resonant signal, we find that $\alpha$ $>>$ $\beta$ and have therefore corrected the oscillations.  Two-laser PLE with no observable oscillations were assumed to have $\alpha$ $<<$ $\beta$ and have not been corrected.  

 This correction is applied in Fig.~\ref{FigOscillationCorrection}. First the off-resonant or background region is differentiated from the on-resonant or peak region.  The background region is then linearly corrected and fit using a sine function with a period of 0.18\,meV (Fig.~\ref{FigOscillationCorrection}a). 
 From this fit the phase of  $P_\mathrm{A} / P_\mathrm{B}$ is obtained, so our correction factor is determined. The resulting $P_\mathrm{A} / P_\mathrm{B}$ can be compared to PLE intensity to check that the oscillations align well with the low energy portion of the data, which was considered part of the background (Fig.~\ref{FigOscillationCorrection}b). Only the period and phase of $P_\mathrm{A} / P_\mathrm{B}$ is checked at this stage. Using the determined $P_\mathrm{A} / P_\mathrm{B}$, the PLE intensity is multiplied by the correction factor.  The effect of this correction can be seen in Fig.~\ref{FigOscillationCorrection}c and Fig.~\ref{FigOscillationCorrection}d.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% next section %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\FloatBarrier
\clearpage
\section{Resonant Excitation}
\label{Sec:Res_Ext}
Fig.~\ref{FigResonantExcitation} displays photoluminescence spectra within the two electron satellite (TES) and longitudinal optical (LO) phonon replica spectral region for a single nanowire and a nanowire ensemble. Spectra were recorded with the excitation laser on- and off-resonance with the In D$^0$-D$^0$X transition. For both, nanowire ensembles and single nanowires, the TES and phonon replica are enhanced in the on-resonance case compared to the off-resonance case. For the nanowire ensemble, a non-specific background can be seen in the on- and off-resonance cases. This non-specific background makes monitoring resonant excitation more challenging for nanowire ensembles. Some single nanowires also show a strong non-specific background similar to the nanowire ensemble. For this study, we screened the dropcast single nanowires for the presence of the non-specific background and only performed two-laser spectroscopy on single nanowires with a negligible non-specific background.

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=5in]{Figures/OnOff_Resonance_TES_PhononReplica.pdf}
  \caption{\label{FigResonantExcitation}
  Photoluminesence spectra of the two electron satellite (TES) and longitudinal-optical (LO) phonon replica spectral region for a single nanowire (bottom black) and the nanowire ensemble (top blue). The ensemble data has been offset for clarity. A dashed line indicates zero intensity for the corresponding data set. All measurements are at 0\,T and 5.2\,K. The excitation power is 7.2\,\textmu W (200\,nW) for the single nanowire (ensemble) measurements. The darker (lighter) data is with the excitation laser on-(off-)resonance with the In D$^0$-D$^0$X peak. A large non-specific background is visible for the nanowire ensemble region for both the on- and off-resonance spectra.
  }
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\FloatBarrier
\clearpage
Fig.~\ref{FigPLE} displays photoluminescence excitation (PLE) spectra recorded on hydrothermally-grown single-crystalline bulk Tokyo Denpa ZnO, a single nanowire, and a nanowire ensemble. For the single crystals, PLE spectra were recorded for the Ga D$^0$-D$^0$X transition; whereas for the single nanowire and nanowire ensemble, the measurements were performed for the In D$^0$-D$^0$X transition. 
The spectral resolution of these scans is well below our laser linewidth of $<$1\,MHz.
The linewidths seen using single-laser PLE measurements at 0\,T are a good indication of the inhomogeneous broadening.
The linewidth observed for the nanowire ensemble is comparable to the linewidth seen for different ZnO bulk crystals, indicating that the inhomogeneous broadening observed for nanowire ensembles is comparable to that of some commercially-available, single-crystalline bulk ZnO. 
The single nanowire (nanowire \#18 from Fig.~\ref{FigPL1}) displays a significantly broadened linewidth, indicating additional inhomogeneous broadening mechanisms as compared to the nanowire ensemble. 
In accordance with the results presented in the main text, we propose strain introduced during the dropcasting process to be the source of this additional inhomogeneous broadening.


\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=5in]{Figures/PLE_Comparison.pdf}
  \caption{\label{FigPLE}
  Photoluminesence excitation (PLE) spectroscopy of bulk samples (purple and red), ensemble nanowire sample (blue), and single dropcast nanowire (nanowire \#18 from Fig.~\ref{FigPL1}) (black). All measurements are performed at 0\,T and 5.2\,K. 
  For the bulk measurements, the excitation laser is scanned over the Ga D$^0$-D$^0$X peak with 100\,nW while the TES and LO-phonon replica luminescence is collected.
  For the single dropcast nanowire measurements, the excitation laser is scanned over the In D$^0$-D$^0$X peak with 7.2\,\textmu W while the TES and LO-phonon replica luminescence is collected.
  For the nanowire ensemble measurements, the excitation laser is scanned over the In D$^0$-D$^0$X peak with 200\,nW. For the nanowire ensemble measurements only,  the non-specific background is subtracted and only the two-LO-phonon replica luminescence is collected. 
  The solid lines are fits to the data. The full width at half maximum (FWHM) for each data set is listed.
  The nanowire ensemble data and the single dropcast nanowire data are reproduced from the main text.
  }
\end{figure}

==> Sec4-OP.tex <==
\section{Optical Pumping/Reverse Spectral Hole Burning}
\label{Sec:OP}
Fig.~\ref{FigOpticalPumpingTES} shows photoluminescence spectra within the two electron satellite (TES) and longitudinal-optical (LO) phonon replica spectral region for a single nanowire under resonant excitation (In D$^0$-D$^0$X) with one or two lasers. The measurements were performed at 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$). The inset in Fig.~\ref{FigOpticalPumpingTES} shows on which transitions the lasers are applied. 
Notably, the signal under two-laser excitation is larger than the sum of the signals obtained for single-laser excitation. 
This is the result of optical pumping. 
Under single-laser excitation, the system is spin-polarized, i.e., the population of electrons is transferred to the ground-state level where no laser field is applied. 
Therefore, in the steady-state, only a small fraction of electrons will remain in the ground-state level the single laser is applied to, and thus a small photoluminescence signal will be recorded. 
In contrast, under excitation with resonant lasers on two different ground state populations, electrons will be pumped back and forth between the ground state levels; therefore, neither ground-state will be fully depleted of electrons and an overall higher photoluminescence signal will be observed.

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=6in]{Figures/Optical_Pumping_TES_PhononReplica.pdf}
  \caption{\label{FigOpticalPumpingTES} 
  Photoluminesence spectra of the two electron satellite (TES) and longitudinal-optical (LO) phonon replica spectral region for a single dropcast nanowire. It is the raw spectra used for the PLE in Fig.~2a of the main text. All measurements are at 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$) and 5.2\,K. 
  Both the pump and probe lasers have an excitation power of 7.2\,\textmu W. The inset shows an energy diagram illustrating the application of the laser fields. The probe laser is on-resonance with the In $\left|\right\uparrow\rangle \Leftrightarrow \left|\right\Downarrow\uparrow\downarrow\rangle$ transition. 
  The pump laser is on-resonance with the In $\left|\right\downarrow\rangle \Leftrightarrow \left|\right\Uparrow\uparrow\downarrow\rangle$ transition. 
  Individually, the pump and probe produce a small signal, because of optical pumping. With both pump and probe on at the same time the signal is greatly enhanced, because population is pumped back and forth between the $\left|\right\uparrow\rangle$ and the $\left|\right\downarrow\rangle$ states.}
\end{figure}
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\FloatBarrier
\clearpage

Fig.~\ref{FigOpticalPumpingEnsemble} displays PLE spectra under resonant single- and two-laser excitation for a nanowire ensemble for the In D$^0$-D$^0$X transition. The measurements were performed at 7\,T ($\hat{c} \parallel \vec{B}, \hat{k}$). The application of the laser fields is shown in the inset of Fig.~\ref{FigOpticalPumpingEnsemble}. Under single-laser excitation, a low signal is observed due to optical pumping (see Fig.~\ref{FigOpticalPumpingTES}). 
Only a feature for the high-energy transition can be observed, indicating optical pumping is more efficient for the low-energy transition. 
The linewidth of the single-laser feature ($\sim$30\,GHz) is a combination of the effects of optical pumping and the ensemble linewidth.
Under two-laser excitation, larger signals are observed due to the re-pumping of population between the two ground spin states. This recovered peak is also called a reverse spectral hole.
The linewidths of the reverse spectral holes (10~-~20\,GHz) are expected to reflect the linewidth of the In D$^0$-D$^0$X transition that is the result of homogeneous broadening mechanisms and broadening mechanisms that are fast compared to our measurement time ($\sim$20\,s). 
Notably, the corresponding linewidths seen for single nanowires (see Fig.~\ref{FigOpticalPumpingOtherNW} and Fig.~2~(a) in the main text) are significantly wider, indicating an additional broadening mechanism affecting the linewidth of reverse spectral holes observed in single nanowires. Such mechanisms may be related to the higher excitation powers used for single nanowires. 

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=6in]{Figures/Optical_Pumping_Ensemble.pdf}
  \caption{\label{FigOpticalPumpingEnsemble} 
  In D$^0$-D$^0$X PLE spectra of an ensemble of nanowires at 5.2\,K and 7\,T ($\hat{c} \parallel \vec{B}, \hat{k}$) with no pump (black), pump on the high energy transition (red), and pump on the low energy transition (blue). The inset shows an energy diagram illustrating the application of the laser fields. The excitation power is 200\,nW for both pump and probe lasers. The solid lines are fits to the data. The two-laser datasets (red and blue) are offset for ease of comparison.}
\end{figure}
  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\FloatBarrier
\clearpage

Fig.~\ref{FigOpticalPumpingOtherNW} displays PLE spectra under resonant single- and two-laser excitation for a single nanowire (nanowire \#41) for the In D$^0$-D$^0$X transition. The measurements were performed at 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$). The application of the laser fields is shown in the inset of Fig.~\ref{FigOpticalPumpingOtherNW}. 
Under single-laser excitation, a low signal is observed due to optical pumping (see Fig.~\ref{FigOpticalPumpingTES}). Only a feature for the high-energy transition can be observed, indicating optical pumping is more efficient for the low-energy transition. 
The linewidth of the single-laser feature ($\sim$60\,GHz) is a combination of the effect of optical pumping and the ensemble linewidth.
Under two-laser excitation, larger signals are observed due to the re-pumping of population between the two ground spin states. This recovered peak is also called the reverse spectral hole.
The linewidth of the reverse spectral hole ($\sim$50\,GHz) is expected to reflect the linewidth of the In D$^0$-D$^0$X transition that is the result of homogeneous broadening mechanisms and broadening mechanisms that are fast compared to our measurement time ($\sim$20\,s).
However, significantly narrower linewidths are observed for the reverse spectral holes in the nanowire ensemble (see Fig.~\ref{FigOpticalPumpingEnsemble}), indicating that there are additional mechanisms contributing to the width of the reverse spectral hole in the single nanowires. Such mechanisms may be related to the higher excitation powers used for single nanowires and would therefore include power broadening, spectral diffusion that is fast compared to our measurement time, and laser-induced temperature broadening. 

\begin{figure}[h]
  \centering
  \includegraphics[width=6in]{Figures/Optical_Pumping_OtherNW.pdf}
  \caption{\label{FigOpticalPumpingOtherNW} 
    In D$^0$-D$^0$X PLE spectra of single dropcast nanowire \#41. This is a different nanowire from the one shown in the main text. Measurements are performed at 5.2\,K and 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$) with no pump (black) and the pump on the high energy transition (blue). The inset shows an energy diagram illustrating the application of the laser fields. The excitation power is 7.2\,\textmu W for both pump and probe lasers. The solid lines are fits to the data. The two-laser data (blue) is offset for ease of comparison.}
  \end{figure}



%=============================== 
Fig.~\ref{Fig_OP_DiffToptica} shows two-laser PLE for a single nanowire with different pump laser wavelengths near the In D$^0$-D$^0$X transition. The measurements were performed at 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$). Fig.~\ref{Fig_OP_DiffToptica}a is a PLE with the pump laser on-resonance with the In $|\downarrow\rangle \Leftrightarrow |\Uparrow\uparrow\downarrow\rangle$ transition. Fig.~\ref{Fig_OP_DiffToptica}(b-g) are PLE with the pump laser shifted by the indicated energy. By comparing the shifted data (blue data) with the on-resonance data (black fit reproduced in each figure), we can see that as we go further off resonance the signal decreases and the linewidth increases. 
This further confirms that the two-laser recovered peak (reverse spectral hole peak) is related to the In D$^0$X transition resonance and thus the re-pumping of population is between the two In D$^0$X ground spin states.

\FloatBarrier
\clearpage

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=5.3in]{Figures/Figure_OP_DifferentToptica.png}
  \caption{\label{Fig_OP_DiffToptica} 
  Two-laser photoluminesence excitation (PLE) spectroscopy of a single dropcast nanowire. All measurements are performed at 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$) and 5.2\,K. All laser powers are 7.2\,\textmu W. The probe laser is scanned over the In $|\uparrow\rangle \Leftrightarrow |\Downarrow\uparrow\downarrow\rangle$ transition while the two electron satellite (TES) and longitudinal-optical (LO) phonon replica luminescence is measured. (a) The pump laser is on-resonance with the In $|\downarrow\rangle \Leftrightarrow |\Uparrow\uparrow\downarrow\rangle$ transition. The black line is a fit to the data. (b-g) The pump laser is shifted from the resonance by the indicated amount. The red line is a fit to the data. The black line is the fit from (a) re-plotted to aid comparison. (g) The pump laser was detuned far enough that no re-pumping was allowed; therefore, the signal was below the noise floor.
  }
\end{figure}


==> Sec5-MagnetoPL.tex <==
\section{Polarization-dependent photoluminescence at magnetic field}
\label{Sec:MagnetoPL}

Photoluminescence measurements were performed on a nanowire ensemble at 7\,T ($\hat{c} \perp \vec{B}$ and $\hat{c} \parallel \hat{k}$) using laser excitation at 3.4440\,eV, i.e., using laser excitation above the band gap of ZnO. At 7\,T, the spin degeneracies of the In D$^0$-D$^0$X system are lifted and four transitions can be detected (see inset of Fig.~\ref{FigMagPLEnsemble}a). For this measurement geometry, the transitions display linear polarizations, whereby two transitions are polarized horizontally and two transitions are polarized vertically. A half-wave plate in the collection and excitation path in combination with a linear polarizer in the collection path (set to V) were used to measure the polarization dependence of the photoluminescence spectra and the results are displayed in Fig.~\ref{FigMagPLEnsemble}. We assume that the polarization of the excitation has no major effect, and that the main effect of the half-wave plate in combination with the linear polarizer is to select which transitions are collected (either H or V).

The left panel of Fig.~\ref{FigMagPLEnsemble}a shows two distinct peaks; their separation is a result of the electron Zeeman splitting. The right panel of Fig.~\ref{FigMagPLEnsemble}a shows a zoomed-in spectra of the high-energy peak. The black and teal arrows indicate the observed shift in peak maximum with polarization; this shift is a result of the hole Zeeman splitting. Fig.~\ref{FigMagPLEnsemble}b shows the full polarization dependence of the peak maxima. Notably, the high-energy peak displays a more pronounced polarization dependence compared to the low-energy peak.

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=7in]{Figures/Magneto_PL_Ensemble.pdf}
  \caption{\label{FigMagPLEnsemble} Polarization-dependent photoluminescence measurements were performed on a nanowire ensemble at 7\,T ($\hat{c} \perp \vec{B}$ and $\hat{c} \parallel \hat{k}$) and 6.3\,K using laser excitation at 3.4440\,eV and 40\,nW. 
   (a) Photoluminescence spectra are shown for two different positions of the half-wave plate. Left panel: Two distinct lines are observed originating from In D$^0$X transitions involving the split ground-states. The lines are denoted as low-energy and high-energy peak. Right panel: A zoomed-in version of the left panel is shown to demonstrate the shift observed in the high-energy peak for different polarizations; this shift originates from the splitting of the excited state of the In D$^0$-D$^0$X system. The arrows indicate the spectral maximums of the transitions shown with the same color. The inset illustrates the different transitions and their polarizations. H (V) stands for horizontally (vertically) polarized light. (b) The relative change in the position of the low- and high-energy peak seen in (a) as a function of the angle of the half-wave plate is displayed. The position of the low- and high-energy feature seen in (a) was determined using a voigt fit. The data points marked in purple and blue correspond to the spectra displayed in (a). Polarization selectivity is observed. 
  }
\end{figure}

The data shown in Fig.~\ref{FigMagPLEnsemble}b can be modelled with $$E_\mathrm{pos, i} = E_\mathrm{center, i} + \Delta E_\mathrm{excited, i}\times\sin\left(a_\mathrm{i}\varphi + b_\mathrm{i}\right) \quad \text{(i = low, high)},$$
where $E_\mathrm{pos, i}$ is the position of the low-energy (i = low) or high-energy peak (i = high). $\varphi$ is the angle of the half-wave plate. $a_\mathrm{i}$ and $b_\mathrm{i}$ are the frequency and phase of the sinusoidal curve. The period of the oscillation is expected to be 90\,$^{\circ}$~\cite{wagner2009gvb}, in accordance with the data shown in Fig.~\ref{FigMagPLEnsemble}b. $E_\mathrm{center, high} - E_\mathrm{center, low}$ equals the ground-state splitting, and thus
$$E_\mathrm{center, high} - E_\mathrm{center, low} = g^\mathrm{\perp}_\mathrm{e}\mu_\mathrm{B}B,$$
where $g^\mathrm{\perp}_\mathrm{e}$ is the $g$-factor of the electron in the geometry used for measurements, $\mu_\mathrm{B}$ is the Bohr magneton, and $B$ denotes the applied magnetic field. With the values stated in Fig.~\ref{FigMagPLEnsemble}b, we obtain a value of 1.91 for $g^\mathrm{\perp}_\mathrm{e}$. $\Delta E_\mathrm{excited, i}$ (i = low, high) represents the splitting of the excited state, and thus can be used to calculate the hole $g$-factor $g^\mathrm{\perp}_\mathrm{h}$ via
$$\Delta E_\mathrm{excited, i} = g^\mathrm{\perp}_\mathrm{h}\mu_\mathrm{B}B.$$
From Fig.~\ref{FigMagPLEnsemble}b, it can be seen that $\Delta E_\mathrm{excited, low}$ is lower than $\Delta E_\mathrm{excited, high}$, indicating that the high energy peak displays better polarization selectivity. Thus, $\Delta E_\mathrm{excited, high}$ can be used to determine a value of 0.05 as a lower bound for $g^\mathrm{\perp}_\mathrm{h}$. These values obtained for the nanowire ensemble are consistent with the values obtained in the main text for a single dropcast nanowire.

==> Sec6-CPT.tex <==
\section{Coherent Population Trapping}
\label{Sec:CPT}
Fig.~\ref{FigCPTOtherNW} shows a high-resolution PLE spectrum under two-laser resonant excitation for the In D$^0$-D$^0$X transition. The measurements were performed at 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$). The application of the laser fields is shown in the inset of Fig.~\ref{FigCPTOtherNW}. Due to the effect of two-laser optical pumping a broad peak with a linewidth of $\sim$40\,GHz can be seen (see Sec.~\ref{Sec:OP} and Fig.~\ref{FigOpticalPumpingOtherNW}). A sharp dip with a linewidth of around 2\,GHz can be seen in the center of the peak, indicating the occurrence of coherent population trapping. The measurements shown here were performed on a different single nanowire (nanowire \#41) than the one shown in the main text.

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=6in]{Figures/CPT_OtherNW.pdf}
  \caption{\label{FigCPTOtherNW} 
   High resolution, two-laser In D$^0$-D$^0$X PLE spectrum of single drop-cast nanowire \#41. This is a different nanowire from the one shown in the main text. The inset shows an energy diagram illustrating the application of the laser fields. Measurements are performed at 5.3\,K and 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$). The excitation power is 7.2\,\textmu W for both pump and probe lasers. The solid lines are empirical fits to the two-laser optical pumping peak and the coherent population trapping dip.
  }
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\FloatBarrier
\clearpage
The left panel of Fig.~\ref{FigCPTPowerOtherNW} shows PLE spectra recorded around the dip seen in Fig.~\ref{FigCPTOtherNW} (nanowire \#41). The measurements were performed at 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$). The application of the lasers fields is indicated in the inset of the right panel of Fig.~\ref{FigCPTPowerOtherNW}. Measurements were performed at different powers for the pump lasers (7.2, 3.6, 0.4\,\textmu W). The right panel of Fig.~\ref{FigCPTPowerOtherNW} displays the linewidth of the CPT dip determined from an empirical Voigt fit. The linewidths observed on this single nanowire are similar to the CPT linewidths observed for the single nanowire discussed in the main text.

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=6in]{Figures/CPT_Power_OtherNW.pdf}
  \caption{\label{FigCPTPowerOtherNW}  
   Left panel: High resolution, two-laser In D$^0$-D$^0$X PLE spectra of single dropcast nanowire \#41 zoomed in on the coherent population trapping dip. This is a different nanowire from that shown in the main text. Measurements are performed at 5.3\,K and 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$). The excitation power is 7.2\,\textmu W for the probe laser. The pump laser power is 7.2, 3.6, and 0.4\,\textmu W. The solid lines are empirical Voigt fits. 
   Right panel: The fit full width half maximum as a function of pump power. The inset shows an energy diagram illustrating the application of the laser fields.
  }
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\FloatBarrier
\clearpage
Fig.~\ref{FigCPTDip} shows PLE spectra recorded under two-laser excitation for the same single nanowire that is discussed in the main text. The measurements were performed at 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$). The probe laser was scanned across the same transition as indicated in the inset of Fig.~\ref{FigCPTPowerOtherNW}. The pump laser was applied to the $|\downarrow\rangle \Leftrightarrow |\Uparrow\uparrow\downarrow\rangle$ transition but slightly shifted in energy in order to probe different two-laser resonance conditions, i.e., different values for $\Delta$. From the left panel of Fig.~\ref{FigCPTDip}, it can be seen that the CPT dip as well as the peak of the reverse spectral hole shift when shifting the spectral position of the pump laser. 
The right panel of Fig.~\ref{FigCPTDip} quantitatively compares the shift of the CPT dip and the peak of the reverse spectral hole while changing the spectral position of the pump laser. 
Notably, the CPT shift is nearly one-to-one with the pump laser shift as expected from coherent population trapping. 
Indeed, the difference between the spectral position of the dip and the spectral position of the pump laser is 0.76-0.77\,eV which is consistent with the expected ground-state splitting of 0.77\,eV at 7\,T assuming an electron $g$-factor of 1.90. This indicates that the electron and hole $g$-factors are close to what is expected from literature~\cite{Ding2009cbe, wagner2009gvb} and what is seen in the nanowire ensemble sample in Sec.~\ref{Sec:MagnetoPL}.
The shift of the peak of the reverse spectral hole does not occur one-to-one with the shift of the pump laser's spectral position; therefore, the reverse spectral hole's lineshape is not solely determined by the position of the pump laser, indicating spectral diffusion.

\begin{figure}[!htbp ]
  \centering
  \includegraphics[width=6in]{Figures/CPT_Dip_Position.pdf}
  \caption{\label{FigCPTDip} 
  High resolution, two-laser In D$^0$-D$^0$X PLE spectra of the single drop-cast nanowire from the main text. The blue and black data is reproduced from the main text. All measurements are performed at 7\,T ($\hat{c} \perp \vec{B}, \hat{k}$) and 5.3\,K. All laser powers are 7.2\,\textmu W. 
  The pump laser wavelength is shifted near the In $|\downarrow\rangle \Leftrightarrow |\Uparrow\uparrow\downarrow\rangle$ resonance. The left panel shows the PLE data with arrows indicating the fit peak and dip positions. The right panel shows the peak~(red) and dip~(black) positions as a function of the pump laser shift.
  }
\end{figure}


==> Sec8-Simulation.tex <==
\section{Simulation of light-guiding in a nanowire}
\label{Sec:Simulation}

 
In our single dropcast nanowire measurements, the excited state dephasing, and therefore our linewidths, are power broadened. However, we are unable to use less power in the current geometry because a minimal fraction of the light emitted by a nanowire lying horizontally on a substrate can be collected with an objective located above the nanowire. 


To better understand how light is emitted from the nanowire, we visualize the electric field strength of a dropcast nanowire using finite difference time domain (FDTD) simulation. The defect emission is modeled as three dipole sources oriented in the x, y and z directions at the center of the nanowire. In the left panel of Fig.~\ref{fig:FDTDNW}, The nanowire is simulated as lying on a substrate of 285\,nm SiO$_2$ deposited on Si. The rectangle outlines the cross section (100 nm$\times$1 $\mu$m) of the nanowire and the horizontal lines divide materials with different indices of refraction.
The electric field power has been guided to the ends of the nanowire and most of the energy flows into the substrate instead of the air due to the higher index of refraction. 

 To increase the collection efficiency,  we envision isolating a single standing nanowire on a sapphire substrate and collecting light from the top of the nanowire to vastly enhance the efficiency of light extraction. Simulated in the right panel of Fig~\ref{fig:FDTDNW}, the majority of the electric field power is guided to the ends of the standing nanowire; however, in this orientation the top end of the nanowire is far from the substrate and pointing toward the objective, allowing for a higher collection efficiency. 


\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.6]{Figures/FDTD_NWs.png}
    \caption{Left: Electric field strength of a ZnO nanowire lying on a Si/SiO$_2$ substrate (285\,nm SiO$_2$).\\
    Right: Electric field strength of a ZnO nanowire standing on a sapphire substrate.}
    \label{fig:FDTDNW}
\end{figure}

